DECE: Decision Explorer with Counterfactual Explanations for Machine Learning Models

With machine learning models being increasingly applied to various decision-making scenarios, people have spent growing efforts to make machine learning models more transparent and explainable. Among various explanation techniques, counterfactual explanations have the advantages of being human-friendly and actionable -- a counterfactual explanation tells the user how to gain the desired prediction with minimal changes to the input. Besides, counterfactual explanations can also serve as efficient probes to the models' decisions. In this work, we exploit the potential of counterfactual explanations to understand and explore the behavior of machine learning models. We design DECE, an interactive visualization system that helps understand and explore a model's decisions on individual instances and data subsets, supporting users ranging from decision-subjects to model developers. DECE supports exploratory analysis of model decisions by combining the strengths of counterfactual explanations at instance- and subgroup-levels. We also introduce a set of interactions that enable users to customize the generation of counterfactual explanations to find more actionable ones that can suit their needs. Through three use cases and an expert interview, we demonstrate the effectiveness of DECE in supporting decision exploration tasks and instance explanations.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> content/note/comments.tex <==
%%% -----------------------------introduction------------------------------------

%%% Motivation
% 4. Existing XAI works and their limitations?
%  * train simple models to mimic the origin model globally
%  * approximate local decision boundary with linear models, such as LIME -- closely related to our work
%      -- limitation:
%         * not actionable
% 5. Instead / another approach is counterfactual explanations, 
% 6. What is counterfactual explanations
%  * the definition is different (from Judea Pearl et al.'s)
%  * we apply the definition in \cite{wachter2017counterfactual}
%  * a case of loan repayment prediction
% 7. Benefits brought by counterfactual explanations
%  * **human-friendly** -- supports from philosophy works
%  * answer "why" problem, provide actionable explanations
%  * ?

% To balance the model performance and the model interpretability, 
% a variety of techniques have been designed to provide post-hoc explanations by using simplified models to approximate the accurate model. (...)
%%% limitation: not actionable; local regions

% Among these works, counterfactual explanations have been proved to be useful by describing a "closest possible world", which is to answer the question, "\textit{how could I change the data to get a desired prediction}." 
% For instance, a person submitted a load request but got rejected, an counterfactual explanations could be like
% "\textit{if you earn 500 dollars more each month, your loan request will be approved}."
% Counterfactual explanations are actionable explanations and proved to be human-friendly. Feature importance and dependency analytics based on counterfactual explanations can also bring insights of possible model flaws and biases to model developers.
% make it 生活化, real scenario 
%%% actionable & try to get a global explanation

% For instance, a user got his loan request rejected and expected an answer to the question: "\textit{How (could I make the change) to get the loan approved.}" 
% The second question is asking for \textit{counterfactual explanations} which describe a "closest possible world",

% Feature importance and dependency analytics based on counterfactual explanations can also bring insights of possible model flaws and biases to model developers. % what-if tool



%  global or local post-hoc explanations.
% 8. Current approaches focused on the counterfactual explanations to an individual instance, such as what-if tools
% 9. We extend this idea to counterfactuals to a subset
% 10. By analyzing the subset counterfactuals, we could
%  * locate vulnerable regions 
%  * understand the decision boundary 
%  * diagnose possible flaws and biases

% From the perspective of model understanding, a natural thought is to evaluate whether the knowledge gained from a single instance can be applied to a subgroup of instances. 
% Analyzing the counterfactuals of a subgroup can help model developers and model users understand the model predictions, diagnose possible flaws and biases, and gain supporting evidence for decision making.
% In our work, we focus on classification tasks on tabular data, which are the most common tasks in real world applications.


%%% Challenge
% 11. Challenges in subset counterfactuals visualization
%  * large amount of counterfactuals -- subset analysis
%  * it is non-trivial to involve human factors in the counterfactuals generation  -- counterfactuals
%  * (low-efficient generating algorithms cannot directly support iterative probing)
% There are two technical challenges to analyzing subgroup counterfactuals. The first challenge is how to provide a visualization summary to a large amount counterfactual explanations.
% We designed a table-based visualization with a set of interaction techniques
% to enable users to explore large tables of counterfactual instances.
% Another challenge appears when decision makers want to customize counterfactuals based their preference, such as the mutable attributes and the order of attribute by preference. How to involve these human factors is a non-trivial problem. 
% We designed a batch of interactions to support the customization. 

% Add a paragraph to introduce what we have done in this paper.



%%% Contribution
% 12. our method?
% 13. contributions
%  * a VA system of counterfactual explanations to a subset
%  * two or three cases
%  * ?

%%%%%% Version_2
%%% Motivation -- by-subset explanation
% 1. Existing works focusing on explaining the model decision can be divided to global explanations and local explanations
%  * global explanations: can be applied to the whole dataset
%    limitation: can be too complex --  "can lead to an overly complicated decision pathway that is ripe for human error."
%  * local explanations: by-instance works
%    limitation: how to define locality is a challenging problem; knowledge gained from an instance may not be able to applied on other nearby instances
% 2. Instead we propose a method to provide by-subset explanations, which is to balance the interpretability and the generality
% 3. We apply counterfactual explanations...


%%%%%% Version_3
%%% Motivation -- decision boundary
% 1. A critical task in explainable ML is to understand the model decision boundary
% 2. Decision boundaries are ...
% 3. By understanding the decision boundary, we could 
%   * 
% 4. The challenge is that the non-linear decision boundary is too complex for human to understand
% 5. Existing works, such as LIME, focus on linear approximations to the decision boundary around a data point, which are called attribution.
% 6. However, linear approximations have serious generality problems
% 7. Instead, we try to convey the non-linear decision boundary of a scalable subspace using counterfactual explanations


% Motivation for Counterfactual:
% 1. The motivation from philosophy (The contrary-to-fact conditional).
% 2. Counterfactuals as \textit{actionable} explanations.
% 3. It is natural to consider subjective preferences (user-customized) with counterfactuals.




% Contributions:

% 1. Visual
% Possible challenges from reviewer:
% 1. What is new about our counterfactual approach (compared with the What-If tool)? 
% * User-customized
% * Diversified
% * Subset counterfactual

% 2. Compared with other model understanding / XAI tools, what is the advantages/benefits of our counterfactual-based approach?

% 3. The rationales/motivation of analyzing counterfactuals of data subset?

%%% -----------------------------related works------------------------------------




%%% ---------------------------design requirements---------------------------------

%%% Q1 - (group-level) when and where will the model goes wrong

%%% Q2 - (group-level) does the model make fair and accountable decision to a subgroup of instances
%   after users select a group of "suspicious" instance, how to evaluate these instances and provide insights about possible biases and flaws
% （btw we can design a pipeline about how to do such analytics based on counterfactuals）

%%% Q3 - (instance-level) how certain is the prediction made by the model
%   "How does the difficulty of recourse vary in a population of interest" 
%   "Do the decisions being made sensible?" (sensitive?)

%%% Q4 - (instance-level) how to gain a desired prediction result by modifying the data

% “If xAI is to produce methods that make algorithmic decision-making systems more trustworthy and accountable, the field's attention must shift to the development of interactive methods for post-hoc interpretability that make it easier to contest algorithmic decisions, and facilitate informed dialogue between users, developers, algorithmic systems, and other stakeholders.”

% start with a dataset 
% \begin{enumerate}

%     \item Explore and compare diverse counterfactuals that cover a wide range of possible changes. (\#instance-level, \#diversity)
    
%     \item Identify and refine data subsets of interests. (\#interaction, \#subset) Maybe we can also design some algorithms to suggest subsets based on pre-defined criteria.
    
%     \item Understand the decision boundary via CFs of subsets. (\#visualization, \#subset)
    
%     \item Customize the counterfactuals with user-specified constraints that reflects user preference or real-world restrictions. (\#interaction)
    
%     \item Identify uncertainty in the classification (\#instance)
    
%     \item Diagnose possible flaws and biases(\#subset)
    
%     % \item Identify the most influential points in the training data to a mis-classification.(\#subset)
    
%     \item "Do the decisions being made sensible?" -- a way to convey the prediction uncertainty by showing the distance to the decision boundary \cite{mittelstadt2019explaining}\cite{ustun2019actionable}
    
% \end{enumerate}


%%% ------------------------------methodology-------------------------------------

% 4.1
% Our work is designed for classification tasks and can be easily extended to regression tasks.
% Without loss of generality, we assume that the model is designed for binary classification tasks so the desired prediction is $\sim f_w(x)$. 
% Such a counterfactual example $x'$ can be used to suggest how a decision subject could \emph{act} to achieve his or her goal. 
% To be more actionable, it is sometimes desirable that the generated counterfactual examples are \emph{sparse} and \emph{diverse}. A sparser counterfactual example is more interpretable and actionable by suggesting only a few features to change. Providing diverse counterfactual examples helps users to find a actionable plan that better fits their needs.
% To make our explanations more actionable to end-users (decision-subjects), it is desirable that the generated examples are \emph{proximal}, \emph{sparse}, \emph{diverse}, and \emph(feasible) as discussed in existing works \cite{mothilal2020explaining, karimi2019model}.

% \begin{align}
%     \label{eq:optim}
%     \argmin_{x'} \max_\lambda \lambda L(f_w (x'), y') + d(x, x'),
% \end{align}
% where $L(\cdot, \cdot)$ is a loss function measuring the difference between the prediction of $x'$ and our desired prediction $y'$. Intuitively, by maximizing $\lambda$, we aim to find a $x'$ whose predicted label is close enough to $y'$.
% For classification tasks, $y'$ is the probability of the desired class (with a default value as $0.5$), and we let $L$ be the ranking loss with zero margin. For regression tasks, we use squared error as in the original \autoref{eq:wachter}. For the distance function $d$, we use the Manhattan distance ($L1$ norm) $d(x, x') = \| x - x' \|_1$.


% $$
% \textup{dist\_cat}(\mathbf{c}, \mathbf{x}) = \frac{1}{\|F_{cat}\|} I(\mathbf{c}^f, \mathbf{x}^f)}
% $$


% For categorical features, we use the standard one-hot encoding before feeding them into the model. That is, for each categorical variable $x_i$, which can take $k_i$ different discrete values, we use $k_i$ binary features $d_{i1}, \cdots, d_{ik_i}$ to replace it. However, simply optimizing \autoref{eq:optim} could generate counterfactual examples that invalidate the one-hot encoding.

% To address this issue, we first introduce a regularization term that encourages the one-hot features of a categorical variable sum up to 1:
% $$
% R_d = \frac{1}{m} \sum_{i=1}^m \left|\sum_{j=1}^{k_i}|d_{ij}| - 1\right|,
% $$
% where $m$ is the number of categorical variables.

% Then, after the optimization completes, we assign each categorical variable the value that correspond to the largest binary feature:
% $
% x_i := \argmax_j d_{ij}.
% $
% In this way, we make sure that each categorical variable is valid.

% 4.2

% If there is any specific algorithm/methods that we would use to analyze subgroup/decision boundaries.

% \note{p1: general ideas of subgroup cf: refinable rules for iterative probing}
% \note{p2: formal definition}
% 1. by-instance cfs are useful for end-users to make decision, while their power to provide general knowledge about how model makes decision is limited
% 2. for model developers and model users, cfs can be used to probe model's decision boundaries, because a cf should lie on a decision boundary
% 3. since the model's decision boundary is quite non-linear (complex) directly presenting the cfs against an arbitrary subgroup can be very confusing to users
% 4. thus we aim to provide ... 
% 5. we make two approximations
% 6. first, instead on analyzing an arbitrary subgroup, we define the subgroup as 
% 7. second, we exam the influence of each feature to the model's prediction independently , for example
%  we define the subgroup cf examples along a feature as:
% 8. this definition has two advantages: 
%    1. the explanations in the form of "rules" are human-comprehensible
%    2. the explanation itself can be iteratively refined by the users: it is achieved in a "what-if" analysis
%      the second advantage is also the key feature of our system: compared with other explainable ml techniques, especially rule-based explanations, which are fixed rules, our work allows users to propose their hypothesis of the model's decisions in the form of rules; then the users can verify and refine their hypothesis through subgroup counterfactual examples.

% % In the last section, we introduce how to generate actionable generate CF examples as explanations to the prediction of a single instance, which could guide the decision subjects to take actions.
% CF examples are naturally good probes for model developers and model users to understand the model's decision boundaries because ideal CF examples should lie on the boundary surfaces. (Otherwise, we can always find a more proximal one at the cross of the $\left \langle \mathbf{c}, \mathbf{x} \right \rangle$ vector and the boundary surfaces.) However, instance-level CF examples are limited to help users gain an overall understanding of the model's decision. 
% % Thus, we aim to enable subgroup-level analysis based on counterfactual explanations.
% Thus, we aim to help users to understand model behaviour by analyzing the distribution of CF examples for instances in a subgroup.
%A naive method is to evaluate its performance with metrics, such as accuracy. However, such an approach strongly depends on the testing data distribution, which is limited to detect potential flaws and bias for the new coming data. In our work, we propose a technique to explain the model's predictions on a subgroup by telling how to make shifts to alter the predictions on a subgroup.

% In our first approaches, we find that CF examples against instances in an arbitrary subgroup can be very hard to summarize and confusing to users. This is because that model's decision boundaries are very complex, which are non-linear and described in a high-dimensional space. 
% }{Summarizing CF examples of a subgroup of instances is quite challenging. This is because model's decision boundaries are complex non-linear surfaces in a high-dimensional space.}
% To provide human-understandable explanations for the model's decision on a subgroup, we use two approximation strategies. 
 
% First, instead of analyzing an arbitrary subgroup, we focus on subgroups that can be defined by setting ranges for each feature values, e.g., patients whose Glucose is under 105 and who is under 30 years old. 
% A formal definition is:
%  \begin{equation}
%      S = D \cap X'_1 \times X'_2 \times ... \times X'_k,
%  \end{equation}
% where $D$ is the training dataset and $X'_j$ is the range of feature $j$'s value. Such subgroups have with clear meaning and can be easily defined by users, which is critical for an exploratory analysis. 
 
% Second, for such a subgroup, we examine the influence of each feature on the model's prediction independently.
% It is achieved by generating constrained CF examples.
% Specifically, we want to find CF examples against instances in the subgroup by only allowing one feature $j$'s value to change freely in the domain $X_j$. 
% In contrast, other feature values can only vary in the limited range $X'_j$, as shown in \autoref{fig:subgroup}. For each feature $j$, we generate a set of CF examples against each instance in the subgroup $S$ by solving:
%  \begin{equation}
%      C_j(S) = \underset{\{\mathbf{c_i}\}}{\textup{argmin}} \sum_{\mathbf{x_i}\in S} L(\mathbf{x_i}, \mathbf{c_i}),
% \end{equation}
% \begin{equation}
%      \textup{such that:}\ \mathbf{c_i} \in X'_1 \times X'_2 \times ... \times X_j \times X'_n,
%  \end{equation}
% where the $L$ is the loss function defined as in \autoref{eq:loss}. So for each subgroup, we generate multiple CF example groups $C_j(S)$ for analyzing how each features affects the model's predictions to the subgroup. 

% For simplicity, we generate one CF example for each instance. The diversity and sparsity constraints are not considered. 

% The above definition is designed in view of the comprehensibility and the refinablility of the explanations.

% The exploration of subgroup CF examples is an iterative process. Initially, the user forms a hypothesis about how the model makes decisions in the form of a rule. 
% For example, women whose BMI is 35 and whose Glucose is under 120 are not likely to have diabetes. Then the generated subgroup CF examples help users to verify or guide users to refine the hypothesis. 
% If all of the CF examples are out of the range, it means that the hypothesis is very likely to be valid. 
% Otherwise, for example, with some CF examples lie around $BMI = 35\ \textup{and}\ Glucose = 115$, users may refine the hypothesis to $Glucose < 115$, and the new boundaries should be closer to the real decision boundaries of the model.
% In real world datasets, we may also consider the feasibility of the CF examples. That is to say, some CF examples with extreme values will not be 

%%% --------------------------------system---------------------------------------




%%% -----------------------------evaluation------------------------------------


% Expert Interview (0.5 page)

% Experts: 5 students
% machine learning expertise: 2 students has been working on machine learning related projects for 3 years; the other 3 has one year learning experience
% visualization expertise: all at least two years

% Organization 
% 10 minutes tutorial
% 20 minutes showcase
% 30 minutes let them use and think aloud

% questions:

% feedbacks:
% ml experts (over 3-years ml project experience): 
% pros:
% * potential application domain / generalizability: how to improve our company's cell phone ranks
% * very novel， 能够帮助决定边界，通常，    更让人信服
% * can tell an exact boundary
% * 健康管理建议
% * 具体的instance增强可信度
% * 能够锁定feature更有用
% * 探索过程中保留中间数据非常有用
% * new findings: sparkline 形状的含义

% cons:
% * table view 和 instance view 对应
% * 调节顺序

% model users / data scientists:
% * 能够告诉用户feature对结果的影响，更能给出具体的范围
% * 帮助用户做数据分析
% * 模型偏见问题 -> 让数据分析更平均
% * side-by-side comparison

% cons:
% 不容易将不同颜色的instance - cf联系在一起

% We collect feedback from five graduate students who majored in computer science. Two students work in machine learning research for over three years and have published in the area. The others have about one-year machine learning study experience. We note the first two students as an expert group and the rest as a common group.
% We first introduce \system{} with an example usage scenario. Then the users explore \system{} for 30 minutes. They are encouraged to ask questions and discuss with us during the exploration. Afterward, we collect their feedback on usage experience, suggestions on potential improvements, and how can this tool helps them with their research or daily life.  \looseness=-1

% \textbf{Counterfactual based approach.} The two experts show great interest in the subgroup level analysis with CF examples. One of an expert says ``\textit{the system can not only tell me whether my hypothesis is correct but also provides suggestions for model's decision boundaries.}'' For the common user group, all the three students say that the definition of counterfactual explanations is ``\textit{very easy to understand}''. However, two students are confused with the group-wise counterfactual explanations (r-counterfactuals) at the beginning. After 10 minutes exploration with the \textit{table view}, they begin to  find it actually quite intuitive.  \looseness=-1

% \textbf{Visualization design.} One student says she likes the design of two align histograms to show the  ``opposite'' groups. However, another students says that at the beginning she mentally connects the bars with the same color together. It takes her a few minutes to connect the original instances with the CF examples. All students think that the \textit{instance lens} in the \textit{table view} and the \textit{instance view} are very useful to support the conclusion with concrete instances. One student from the expert group says that keeping a list of subgroups is  useful. With this function, she can quickly recall  a previous step in the exploration.  \looseness=-1

% % \textbf{Usage Scenario.} When asked about what you will do with \system{}, students in the both two groups give diverse answers. A student in the common user group says that she wants to use \system{} to get suggestions for keeping a good health. 
% % Another student who is an intern at a tech company says that he wants to suggest his manager to use this system. ``\textit{He may find good market strategies to help our product to reach to a higher ranking.}''
% % In the expert group, one student suggests that \system{} can be used to detect model bias.

% \textbf{Suggestions for improvements.} One student in the expert group suggests that in the subgroup level analysis, we may directly show users with an optimized solution to refine the subgroup.  \looseness=-1
% One student in the common user group suggests that the shape of the sparkline in each cell may 


%%% -----------------------------discussion------------------------------------


% \section{Conclusion}

% In this work, we introduce \system{}, a model-agnostic, counterfactual explanation-based approach to help users explore and understand a machine learning model's decision. Our system supports three types of users: decision makers, model developers, and decision subjects. The visual interface supports iterative probing the decision boundaries of any model by analyzing subgroup counterfactuals as well as generating actionable examples by interactive imposing constraints on possible feature variations. Three example usage scenarios on datasets from different application domains, including finance, education, and healthcare, demonstrate the effectiveness of the proposed approach.

% \textbf{Scalability of the Visualization.} The current design of the\textit{ table view} can visualize nine subgroup rows or about one thousand instance rows (one takes a pixel vertically) on a typical laptop screen with 1920 $\times$ 1080 resolution. Users can find those out-of-screen subgroups and instances by scrolling. Users can also adjust the width of each column by dragging the boundaries. They can also collapse the features they are not interested in and inspect the details of a feature by increasing the column width. In most cases, about ten columns can be displayed in the table, as shown in the first and second usage scenario.

% \textbf{Generalizability and Scalability of the Counterfactual Generation Engine.} The generation algorithm is a gradient-based approach to optimize the CF examples, which works for all differentiable models. Generating CF examples for non-differentiable models (\eg~decision trees) is an active research topic in the machine learning community \cite{lucic2019actionable}. Since the counterfactual generation engine should be able to support timely interactions with users, the running time is also an important factor for improving user experience. We use mini-batch to speed up the generation process and test the efficiency of our algorithm on four datasets, including Pima Indian Diabetes Dataset (768 instances), German Credit Dataset (1000 instances), Graduate Admission Dataset (500 instances), and HELOC Dataset (10459 instances). The running time to generate counterfactual examples for the entire dataset is ~2 seconds for Pima Indian Diabetes Dataset and Graduate Admission Dataset and ~10 seconds for the other two. We expect that by parallelizing the CF generation process, significant speedup could be achieved.

% \textbf{Feedback from Decision Makers using ML Model} We currently don't have feedback from real decision makers, which is one of our major target users. We expect to deploy our system in real-world applications and collect feedback on long term usage. 
